ViFi-Loc: Multi-modal Pedestrian Localization using GAN with Camera-Phone Correspondences

In Smart City and Vehicle-to-Everything (V2X) systems, acquiring pedestrians' accurate locations is crucial to traffic safety. Current systems adopt cameras and wireless sensors to detect and estimate people's locations via sensor fusion. Standard fusion algorithms, however, become inapplicable when multi-modal data is not associated. For example, pedestrians are out of the camera field of view, or data from camera modality is missing. To address this challenge and produce more accurate location estimations for pedestrians, we propose a Generative Adversarial Network (GAN) architecture. During training, it learns the underlying linkage between pedestrians' camera-phone data correspondences. During inference, it generates refined position estimations based only on pedestrians' phone data that consists of GPS, IMU and FTM. Results show that our GAN produces 3D coordinates at 1 to 2 meter localization error across 5 different outdoor scenes. We further show that the proposed model supports self-learning. The generated coordinates can be associated with pedestrian's bounding box coordinates to obtain additional camera-phone data correspondences. This allows automatic data collection during inference. After fine-tuning on the expanded dataset, localization accuracy is improved by up to 26%.

==> discussion.tex <==
\section{Discussion}
\textcolor{red}{Marco's comment (2). How large is the network? how much computation it takes? }

% \textcolor{red}{Marco's comment (3). example of how this tech can be used in practice, what is the practical scenario once the network is trained? how it the network deployed? Reasonable? feasible?}

\textbf{potential use case} This localization refinement can be used in smart intersection where pedestrian's locations can be fetched and refined by the the road side unit (RSU) that is equipped with an RGBD camera and a WiFi access point. A pedestrian can choose to opt into this location refinement service so that its smartphone would exchange messages with the WiFi access point and provide the system with its phone data including FTM, IMU and GPS measurements. At the RSU's side, the deployed network will make inference on the received phone data to produce a refined GPS location and send this location back to the user's smartphone. At the same time, the produced 3D coordinates will be used to associate with camera observed pedestrian's local 3D coordinates to obtain more data correspondences for future training. 

==> overview.tex <==
\section{Overview}
\begin{figure}[]
    \centering
    \includegraphics[width=0.42\textwidth]{fig/overview_v3.pdf}
    \caption{Overview figure }
    \label{fig:overview}
\end{figure}
In this paper we propose a cross-modal prediction mechanism that generates a location estimation in the camera modality based on wireless measurements. We introduce a Generative Adversarial Network (GAN) architecture to learn the correlation and linkage between the a person's camera modal measurement and wireless modal measurement. The network is capable of predicting a person's accurate location coordinates with respect to the camera coordinate reference system based on her wireless measurement. 

The first part of this work focuses on training and testing the proposed GAN architecture.  During training phase, measurements of a pedestrian's multi-modal data within a time window will be fed into the network. Specifically, measurements from the wireless modality includes WiFi FTM, IMU sensor data and smartphone GPS readings; Measurements from the camera modality include bounding box centroids and depth measurement. Although wireless measurement and camera measurement are not directly comparable, they both describe and encode a pedestrians's walking trajectory and gait information. To reflect this intuition, the network first extract representative features from input measurements and enforce the extracted features to be close to each other in the hyper-space via the embedding loss. Then a decoder is applied to the feature vector from wireless modality to generate a location estimation with respect to the camera coordinate frame. The generated coordinate will be judged by a discriminator with the GAN loss to ensure that the coordinate prediction is within the same distribution of the true locations. 

The second part of this work is focusing on making the system to work at scale. Training the proposed network require multi-modal data correspondences from one or more experiment participants. To Obtain such data correspondences, one option is to collect a single participant's multi-modal data. Another option is to collect multiple participants' data and obtain the data correspondence through post processed data association. Either of these options is time and resource consuming. Here we propose a semi-supervised approach that leverage the network output to automatically produce more multi-modal data correspondences to facilitate larger scale training. Upon obtaining the estimated locations from pedestrian's wireless measurement, we perform data association within the camera modality by comparing the predicted location coordinates with the existing bounding box centroids 3D locations. Since each predicted location corresponds to a pedestrian's measurement, associating the predicted location with camera modality measurement is equivalent to obtaining multi-modal data correspondence for a pedestrian. After this we can use the associated correspondences as new data samples. The semi-supervised approach allows us to easily obtain large scale reliable training data without dedicated participant employment and data collection.
